Scaling the Scattering Transform: Deep Hybrid Networks

We use the scattering network as a generic and fixed ini-tialization of the first layers of a supervised hybrid deep network. We show that early layers do not necessarily need to be learned, providing the best results to-date with pre-defined representations while being competitive with Deep CNNs. Using a shallow cascade of 1 x 1 convolutions, which encodes scattering coefficients that correspond to spatial windows of very small sizes, permits to obtain AlexNet accuracy on the imagenet ILSVRC2012. We demonstrate that this local encoding explicitly learns invariance w.r.t. rotations. Combining scattering networks with a modern ResNet, we achieve a single-crop top 5 error of 11.4% on imagenet ILSVRC2012, comparable to the Resnet-18 architecture, while utilizing only 10 layers. We also find that hybrid architectures can yield excellent performance in the small sample regime, exceeding their end-to-end counterparts, through their ability to incorporate geometrical priors. We demonstrate this on subsets of the CIFAR-10 dataset and on the STL-10 dataset.

==> caltech101.tex <==
We study briefly the property of our SLE descriptor with spatial window size $16^2$, without any ad-hock spatial localization component, such Spatial Pyramid Poolin. Caltech101 is a simple dataset constituted by 9144 samples, and 102 classes. We followed the standard procedure\cite{} with 10 folds and studies the per class accuracy, with 30 training samples per class, using a linear SVM. Applying our raw scattering network leads to an accuracy of $62.8\pm0.7$, and the outputs features from $F_1,F_2,F_3$ brings respectively an absolute improvement of $13.7,17.3,20.1$ respectively as suggested in \cite{oyallon,fergus}. The accuracy of our SLE descriptor is thus $82.9\pm0.4$, which is about the same level as \ref{fergus}. However, the receptive field of \cite{fergus} is quite larger, which means the CNN is likely to build invariance to translation larger than $16$. More work to understand the property of the SLE descriptor should be done, as its locality makes it an ideal candidate for task such image retrievial, yet this is not the purpose of this paper.

==> imagenet_cifar_full.tex <==
%We compare our algorithm to supervised, unsupervised and semi-supervised deep networks and evaluate them on the CIFAR10, STL10 datasets and Imagenet ILSVRC2012 datasets. CIFAR10 datasets consist of colored images of size $32\times32$, with  50000 images in the training set, and 10000 in the test set, divided in 10 classes. The RGB channels of the image are simply standardized.
We evaluate the Shared Local Encoder on the Imagenet ILSVRC2012.  Imagenet is a challenging natural color images dataset. It consists of $1.2$ million training image and $50000$ validation images, divided into $1000$ classes.  %the use of a hybrid architectures using the Imagenet ILSVRC and CIFAR-10 datasets. We first consider the completely local encoded based architecture described in \ref{sec:TBD_ARCH}. This not only allows us to demonstrate that the scattering representation can be used without \textcolor{red}{learned convs>1} to achieve accuracies comparable to the famed AlexNet \cite{} and superior to the hybrid architecture of \cite{Perronin}.

%Imagenet 2012 is a challenging dataset as it is large and has many variabilities. Indeed, there are 1.2M(TO CHECK) natural color images in the training set and a validation set of about 500k images. There are 1000 corresponding classes. No specific prepreocissing is applied to the image.

%In all our experiments unless otherwise stated we use the wavelet parameters and the discretization from \citep{oyallon2015deep}.
\if false
\section{Feature Encoding for Scattering performs well on Imagenet}
We use a simple neural architecture which does not utilize any convolutions \textcolor{red}{need good prefix} to demonstrate the discriminability properties of the scattering transform. We note that our method is comparable to that of \cite{perronnin2015fisher} in that it does not utilize any of the standard convolutional network components, but relies simply on a feature encoding followed by convolutional layers. Indeed despite the simplicity we obtain an accuracy comparable to that of the famed AlexNet architecture, while relying on a more interpretable feature representation. 

We use the following architecture consisting of a 3 layer neural network that encodes the scattering representation\textcolor{red}{need good word for scattering features in spatial} followed by a fully connected layer applied directly on the feature encoding (not taking into account the position). The 3 layer encoding can be implemented using a stack of 1x1 convolutions which are followed by the 2 FC layers.
\fi





\subsection{Shared Local Encoder on Imagenet}

\begin{figure}
\begin{center}
\begin{tikzpicture}
\node at (0,0) [minimum width=1cm,line width=0] (x) {$Sx(u)$};
\node at (0,0.6) [minimum width=1cm,line width=0] (x) {$Sx(u)$};
%\node at (0,0) [minimum width=2cm,line width=0] (x) {Input};
%\node at (0,0.7) [minimum width=1.6cm,draw,align=center] (W1) {\small $F_1$};
%\node at (0,1.4) [minimum width=1.6cm,draw,align=center] (W2) {\small $F_2$};
\end{tikzpicture}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Imagenet architecture}
\label{fig:short}
\end{figure}


\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
\bf Method  &\bf Top 1 &\bf Top 5  \\
\hline\hline
\small \bf   Scattering hybrids    \\
\hline
Scat + SLE  & 43.0 &20.4 \\

\hline
\small \bf  Unsupervised       \\
\hline
FV + 3 FC       &44.4  & 21.6 \\
FV + SVM         & 45.7 & 25.7 \\
\hline
\small \bf  CNNs       \\
\hline
AlexNet  & 43.1 & 19.9\\
%GoogleNet& 32.8&11.0\\
\hline
\end{tabular}
\end{center}
\caption{Top 1 and Top 5 percentage error reported from one single crop on ILSVRC2012.}
\end{table}

We introduce the architecture of our Shared Local Encoder (SLE) and describe its performances on ILSVRC2012. We first describe our training pipeline, which is similar to \cite{zagoruyko2016wide}. We trained our network for 90 epochs to minimize the neg log cross entropy loss, with a SGD using momentum 0.9 and batch size of 256. We used a weight decay of $1\,10^{-5}$. The initial learning rate is $0.1$, and is dropped off by $0.1$ at epochs $30,50,70,80$. During the training process, each image is randomly rescaled, cropped, and flipped as in \citep{NiN}.The final crop size is $224\times 224$. At testing, we rescale the image to a size of 256, and extract a center crop of size $224\times 224$. 

We use an architecture which consists of a cascade of a scattering transform, a Supervised Local Encoder $f$, followed by fully connected layers. Figure \ref{} describes our architecture. We select the parameter $J=4$ for our Scattering network, which means the output representation has size $14\times 14$ spatially 1251 in the channel dimension. $f$ is implemented as 3 layers of 1x1 convolutions of size 1024. There are 2 fully connected layers of size 1524. For all learned layers we use batch normalization followed by a ReLU \cite{alexnet} non-linearity. Since we observed that the Scattering features can suffer from a bad conditionning, we also apply a batch normalization at the ouput of the Scattering network, with a  momentum equal to 0.9.

Table \ref{bullshit} reports our numerical accuracies obtained with a single crop at testing, compared to other analogous models, several of them corresponding to state-of-the-art approaches in 2012. We obtain 20.4\% at Top5 and 43.0 top 1. The performance is analogous to the network from \cite{krizhevsky2012imagenet}. Our hybrid model is analogous, and comparable to that of \cite{sanchez2011high,perronnin2015fisher}, SIFT features encoded via a Fisher Vector (FV) \cite{init author} are extracted.  Observe this is an unsupervised representation. Two approaches are then used: either the  spatial localization is handled either by a Spatial Pyramid Pooling \cite{créateur}, which is then fed to a linear SVM \cite{SVM}, either the spatial variables are directly encoded in the FVs, and classified with a stack of three fully connected layers. This last method is a major difference with ours, as the obtained descriptor does not describe a local spatial neighrborhood  anymore. Furthermore, in both case, the SIFT are densely extracted which correspond to approximatively $XXX$ descriptors, whereas in our case, only $14^2=$ scattering features are extracted. Indeed, we tackle the non-linear aliasing via random cropping that corresponds to linearization of small translations. In Top1, \cite{peronnin,dsq} obtain respectively BULSHIT and BULLSHIT. Our method brings an improvement of BULLSHIT and BULLSHIT.

AlexNet obtains a Top1 accuracy of 43.1 single-crop accuracy, which is nearly equivlent to our 43.0 of our SLE network. The AlexNet has 8 layers and as early as the second layer, the receptive field at a given spatial position corresponds to an area of $30 \times 30$ of the original input image. Contrary to our training pipeline that consists in 5 learned layers with constant receptieve field of size $16 \times 16$, except for the fully connected layers that build a global representation. This is a surprising result, as it seems to suggest context information is only necessary at the very last layers, to reach AlexNet accuracy.



%We use the supervised encoding of the scattering coefficients described in Section ~\ref{} trained jointly with 2 fully connected layers as the classifier to demonstrate \textcolor{red}{one word summery of what we show?}. We note that our method is comparable to that of \cite{perronnin2015fisher} in that it does not utilize any of the standard convolutional network components, but relies simply on a feature encoding followed by a standard neural network. The difference lies in that \cite{perronnin2015fisher} extracts very dense features, of size \textcolor{red}{number},  and \textcolor{red}{incomplete? ed one word here to describe Scatter>SIFT} at each spatial location, and uses an unsupervised encoding (Fisher Vectors),   Indeed despite the simplicity of the encoding and classifier on top of the scattering network we obtain an accuracy comparable to that of the famed AlexNet architecture, while using a more interpretable feature representation. 
\if False
We use 1x1 convolutional layers of size X and 2 FC layers of size Z network. The final validation error is shown in Figure \ref{} and compared to several standard architecutres. We see that it substantially outperforms the result of \cite{perronnin2015fisher} and obtains an accuracy very close to that of \cite{krizhevsky2012imagenet}. 

\textcolor{red}{
WE NEED TO SHOW A DIFFERENCE WITH THE PIPELINE OF PERRONNIN IS THE DENSITY OF THE EXTRACTION OF THE SIFT, THE SUPERVISION, WE NEED TO ADD FIGURE WITH THE ALGORITHM, TO EXPLAIN WHY WE DO DATA AUGM(justifi is CIFAR with local translations that are linearized and aliasing of the representation), THE DIFFERENCE THAT FV INTERNALLY INCORPORATE THE LOCAL SPATIAL POSITION, WE DON'T,  SHOW THAT NO BODY CAN DO 1x1 EXCEPT WITH SCATTERING, SAY WE ARE HAVE LESS LAYERS, DOING AN ANALYSIS IN TERM OF DEPTH, OF SPEED; WE NEED TO EXPLAIN WHY IT IS USELESS ON THE RAW DATA(eg speed+impossible to discriminate anything)}
\fi

\subsection{Interprating the first layer} %of the Scatter Encodings}\label{simpl}


\begin{figure}
\begin{center}

\includegraphics[width=.9\linewidth]{bullsit.eps} 
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Histogram of  $\hat F_1$ amplitude}
\label{fig:short}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=.9\linewidth]{little_wood.eps} 
\includegraphics[width=.9\linewidth]{little_wood_1d.eps} 
\end{center}
   \caption{Littlehood paley of $F_1$}
\label{fig:short}
\end{figure}


%Many works have studied the Alexnet architectures . The simplicity of our model and the fact that it is built upon allow us to show insights on the nature of the operations required to obtain strong classification performance. 

Finding structure in the kernel of the layers of depth less than $2$ \cite{travail_irene,zeiler2014visualizing} is  a complex task, and few empirical analysis exist that shed light on the structure \cite{oyallon2017} of deeper layers. A scattering transform with scale $J$ can be interpreted as a CNN with depth $J$ \cite{oyallon} \textcolor{red}{?? ... CNN of depth 2 - ED:OUI...}, whose  channels indexes correspond to different scattering path\cite{bruna}, which is a structuration.  \textcolor{red}{This structure is consequently inherited by the first layer of our SLE $f$}. We analyse this first learned layer and show that it builds explicitly invariance to local rotations, yet also that the Fourier bases associated to rotation are natural bases of our operator. \textcolor{red}{I PROPOSE THIS:} It is a promising direction to understand the nature of the two next layers.%Thus to a greater extent than the analogously performing AlexNet the behavior of our SLE network can be understood \textcolor{red}{I wrote it but is it too strong this statement? I like it if not}.

We first establish some mathematical notions linked to the rotation group that we use in our analysis. For the sake of simplicity, we do not consider the roto-translation group.
For a given input image $x$, let $r_\theta . x(u)\triangleq x(r_{-\theta }(u))$ the rotated image by angle $\theta$, which corresponds to  the linear action of rotation on images. Observe the scattering representation is  covariant with the rotation in the following sense:
\[S_1(r_\theta.x)(u,\theta_1)=S_1x(r_{-\theta}u,\theta_1-\theta)\triangleq r_\theta.(S_1x)(u,\theta_1)\]
\[S_2(r_\theta.x)(u,\theta_1,\theta_2)=S_2x(r_{-\theta}u,\theta_1-\theta,\theta_2-\theta)\triangleq r_\theta.(S_2x)(u,\theta_1,\theta_2)\]

Observe that in the case of the second order coefficients, $(\theta_1,\theta_2)$ is covariant with rotations, but $\theta_2-\theta_1$ is an invariant to rotation that correspond to a relative rotation. 

The rotations are a compact group, thus it is possible \cite{complex haarmonic anlasysis book like watman} to define a Fourier transform along rotation, and even  a scattering transform \cite{laurent sifre} along the more complex roto-translation group. Fourier analysis permits the measurement of the smoothness of the operator and is a natural structuring operator in our case: for a function $f:\theta \rightarrow f(\theta)$, we write $\hat f: \omega_\theta \rightarrow \hat f(\omega_\theta)$ its Fourier transform.
%Observe that applying a rotation $r_\theta . x=x(r_{-\theta }u)$ translates the coefficients, ie:


%However, for $S_2x$, the natural set of coordinates that gives a rotational invariant for angles is in fact given by:
%\[\tilde S_2 x(u,\theta_1,\alpha)=S_2x(u,\theta_1,\theta_1+\alpha)\]
%where $\alpha$ corresponds to a relative angle, which naturally leads to:
%\[\tilde S_2(r_\theta.x)(u,\theta_1,\alpha)=\tilde S_2x(r_{-\theta}u, \theta_1-\theta,\alpha)\triangleq r_\theta.(S_2x)(u,\theta_1,\alpha)\]


We numerically analyze the nature of the operations performed along angle variables by the first layer $F_1$ of $f$, with output size $K=1024$. Let us define as $F_1Sx=\{F^0_1S_0x,F^1_1S_1x,F^2_1S_2x\}$ the restrictions of $F_1$ to the order 0,1,2 scattering coefficients respectively. Let $1\leq k \leq K$ an index of a feature and $1\leq c\leq 3$ the color index. In this case, $F^0_1S_0x$ is simply the weights associated to the smoothing $S_0x$ of $x$. $F^1_1S_1x$ depends only $(c,j_1,\theta_1,k)$, and $F^2_1$ depends on $(c,j_1,j_2,\theta_1,\theta_2,k)$. We would like to characterize the smoothness of these operators with respect to the variables $(\theta_1,\theta_2)$, because our representation is covariant to rotations.

To this end, we define by $\hat F_1^1$, $\hat F_1^2$ the Fourier transform of these operators along the variables $\theta_1$ and $(\theta_1,\alpha)$ respectively. Then the operator is expressed in the tensorial Frequency domain. Since those operations are involutive (up to constants and reflexions), one can easily recover the original operator. In this experiment, we normalized each filter of $F$ such that they have a $l^2$ norm equal to 1.

Let  us demonstrate how to sparsify this operator in its frequency basis. We simply threshold  by $\epsilon$ the coefficients of the operators in the Fourier domain, e.g.. we replaced the operators $\hat F_1^1$, $\hat F_1^2$ by $1_{|\hat F_1^1|>\epsilon}\hat F_1^1$ and $1_{|\hat F_1^2|>\epsilon}\hat F_1^2$. Figure \ref{bullshithisto} shows the repartition of the amplitude of $\hat F_1^1,\hat F_2^2$ after this thresholding: $80\%$ of the coefficients are 0 and the amplitude of the coefficients are small. \textbf{Without retraining} our network performs  about $2\%$ worse on Top 1 and Top 5 Imagenet : we proved that this basis permits  a sparse approximation of $F_1$.

We know study the repartition of the selected frequency of our operator. To this end, we introcuce the littlewood paley\cite{} of our operator :
\[\Omega\{F_1\}(\omega_1)=\sum_{k,j_1,c}|\hat{F}^1_1(k,j_1,c,\omega_1|^2\]
\[\Omega\{F_2\}(\omega_1,\omega_2)=\sum_{k,j_1,j_2,c}|\hat{F}^2_1(k,j_1,j_2,c,\omega_{\theta_2},\omega_{\theta_1}|^2\]

It permits to visualize the spectrum of a convolutional operator, and in our case, to quantify the smoothness of our filter.Figure \ref{} permits the analysis of these two quantity. One sees that most of the energy is concentrated in the low frequency domain, which indicates that operator explicitely build an invirant to local rotations.
%In the case of a wavelet transform $W$, this corresponds to the  of the operator, e.g. the spectrum of $W^*W$.
%Before thresholding, all the frequencies were excited. After this operation, approximatively $20\%$ of coefficients are non-zero. We have tested our network without any retraining and observed a negligible loss of accuracy. We proved that this basis permits  a sparse approximation of our filters. Figure \ref{bullshit} shows our operator in its sparse basis. %NEED TO DO A NICE FIGURE WHERE COEFFICIENTS ARE ORGANIZED, EDOUARD WILL DO IT.



%Furthermore, we decided to keep only the two first frequencies of $F_1$ along the variable $\theta_1$, i.e. we replaced the operators $\hat F_1^1$, $\hat F_1^2$ by $1_{|\omega_{\theta_1}|\leq 1}\hat F_1^1$, $1_{|\omega_{\theta_1}|\leq 1}\hat F_1^2$. This results in a loss of accuracy of roughly $5\%$. We then fix the layer $F_1$, and decide to retrain the next layers, keeping the entire training procedure identical again with an initial learning rate of $1$. We obtain a classification accuracy which is $3\%$ below the original architecture. This indicates that the network can almost recover discriminative information from averaged coefficients in angle. SHALL WE DO IT? IT POSSIBLE TO ADD AN ANALYSIS OF THE REPARTITION OF THE FREQUENCIES EXCITED IN ANGLES ALSO

%The first experiment shows that in a natural basis it is possible to sparsify the operator. The last experiment indicates that most of the operations performed by the first layer of our network are smooth since they are localized in the Fourier space.  This is equivalent to first projecting via an angular averaging each scattering coefficient and it suggests that the system autonomously builds an invariant to geometrical variabilities. While this does not prove that nomore geometrical operators are applied in the next layers, but it does show it is possible to obtain a good accuracy ($3\%$ below the original result) with a representation after $F_1$ which is stable to local roto-translation and deformation variabilities, thanks to a roto-translation averaging.


\subsection{Transfering on Caltech 101}
WE WANT TO TRANSFER THAT BULLSHIT SOMEWHERE

%We observe several facts. First, it is possible to threshold the coefficients in this basis without any loss in performances. It leads to a representation with $5\%$ coefficients not sparse, which indicates that we built an operator more regular. Besides, if we set to 0 the high frequency in angles, and retrain the top of this operator, we observe a loss in accuracy of $2\%$. This indicates that the deepnetwork uses mostly the low frequency in angles to recognize images, and thus it is building invariants explcitely to rotation. Observe this is the first time that we can have an interpretation on the third linerar operator of an architecture.
\if false
\subsection{Scattering hurts only a little bit(\textcolor{red}{YEAH TITLE MUST CHANGE BIATCH}}
RESNET RESULTS, EXPLAIN IT SHOWS 
We report the classification accuracies in Table \ref{CIFAR} and discuss them below. We compare our architecture with the unsupervised scattering architecture \citep{oyallon2015deep}. The roto-translation scattering is almost identical to scattering, except that it recombines the channels along the rotation axis by applying a wavelet transform along angles, building more complex geometrical invariants. The classifier of this paper is a RBF SVM kernel, which can be interpreted as a two-layer deep neural network. For the sake of simplicity, we have trained on top of our scattering network a 3 layer fully connected  network with size 2048, similarly to \citep{perronnin2015fisher}. Without data augmentation, the accuracy of the network is respectively $3.7\%$ and $8.9\%$ below the roto-translation scattering on CIFAR10 and CIFAR100. However, applying data augmentation with translation of length less than $2^2$ permits recovering this loss in accuracy, resulting in accuracies of $83.0\%$  and $56.7\%$ (we let the network train for 400 epochs here) respectively on CIFAR10 and CIFAR100. One major difference to our approach is that the system in \cite{oyallon2015deep} uses a large amount of oversampling. This suggests that in order to learn the appropriate features it is necessary to average the small translation displacement; even if the representation is built to be invariant to translation, its construction relies, for fast computation, on an approximative (but justified)  downsampling that leads to non-linear aliasing. 

%With a simple projection, the scattering transform at scale $J=2$ performs $3\%$ worse than the roto-translation scattering transform. This is mainly due to two reasons: a regularization issue, since the images used in [] were oversampled.  Secondly, more invariance in translation were used in this work. Less invariance is necessary to learn an intermediary discriminant representation. 

Applying a supervised convnet significantly improves the accuracy of the scattering with 3 fully connected layers, and  leads to comparable results with other supervised deep  representations: 91.4\% on CIFAR10 and 69.5\% on CIFAR100. We compare our work with the Highway network \citep{srivastava2015training}, that consists in a  deep cascade of 19 linear and non-linear operators, with an extensive data augmentation. Besides, since our convnet is kept as simple as possible, we also compare our architecture to the All-CNN \citep{springenberg2014striving} work. The latter performs slightly better on CIFAR10, but our hybrid network has a better generalization on CIFAR100. This indicates that supervision is essential, but that a geometric initialization of the first layers of a deep network leads to a discriminative representation as well. It is also interesting to observe that we could not find any architecture that was performing worse on CIFAR10 than ours, but better on CIFAR100. Since the number of samples available per class is lower, this could indicate that learning is easier in this case with a scattering initialization. 

A Wide Resnet \citep{zagoruyko2016wide} outperforms our architecture by $4.8\%$ on CIFAR10 and $12.2\%$ on CIFAR100, but it requires more engineering process to be designed and is deeper. It is important to recall that, contrary to the wide Resnet, there are no instabilities due to geometric transformations (e.g. translations or deformations), and that the two first layers which are responsible for a large fraction of the computation are not learned, resulting in computational savings. Obviously, the scattering layers do not suffer from the vanishing or exploding gradient issues.
\fi

